Discovering Useful Compact Sets of Sequential Rules in a Long Sequence

We are interested in understanding the underlying generation process for long sequences of symbolic events. To do so, we propose COSSU, an algorithm to mine small and meaningful sets of sequential rules. The rules are selected using an MDL-inspired criterion that favors compactness and relies on a novel rule-based encoding scheme for sequences. Our evaluation shows that COSSU can successfully retrieve relevant sets of closed sequential rules from a long sequence. Such rules constitute an interpretable model that exhibits competitive accuracy for the tasks of next-element prediction and classification.

==> rulemining.tex <==
We now present our proposed algorithm to mine a compact set of sequential rules using an evaluation criterion inspired from the MDL principle. We call our algorithm \algCossu, short for COmpact Sets of Sequential rUles.
% The rules that should capture the most important regularities observed in a long sequence, and should, therefore compress the sequence optimally. %Such rules are individually and jointly useful: they can by themselves efficiently compress large portions of the sequence and they are not redundant. This last statement implies that the rules do not redo the work that other rules could achieve. 
%We clarify this intuition in the upcoming sections: 
We start the discussion in Section~\ref{subsec:rule-encoding} by explaining how to encode a long sequence of symbols using sequential rules, i.e.\ presenting our encoding scheme. This preamble sets the ground for the description of the \algCossu{} algorithm in Section~\ref{subsec:cossu}.

\subsection{Rule-based Encoding for Sequences}
\label{subsec:rule-encoding}
The application of the MDL principle requires us to define a scheme to encode a long sequence $S$ by means of a model ---a rule table $\mathcal{H}^{\omega}(R)$ in our scenario.
In the following we explain how to encode such a model, and how to use it to encode a long sequence.

\subsubsection{Rule Table Encoding.}
Recall that MDL is a formalism that relies on the notion of compression to quantify the complexity of a model as well as its goodness of fit on the data (Equation~\ref{eq:mdl}). For this reason, a rule table does not need to assign actual codes to rules and symbols, but only compute the optimal length in bits of those codes. Once all code lengths are properly defined, we can use them to estimate the size of the model in bits, i.e., the term $l(\mathcal{H}^{\vec{\omega}}(R))$, and the size of the sequence $S$ when its symbols are replaced by the ``codes'' stored in the rule table, i.e., the term $l(S|\mathcal{H}^{\omega}(R))$. From the definition of a rule table in Section~\ref{subsec:mdl}, it follows that we must encode the antecedent ($S_a$), the succedent ($S_c$), and the optimal code length $\omega$ of each of the rules. We define the marginal code length of a sequence $S' \sqsubseteq S$ by: $$l(S', S) = \sum_{1 \le i \le |S'|}{-p_{_S}(S'(i)) \cdot \mathit{log}(p_{_S}(S'(i))) }$$
In the formula $p_{_S}(\sigma)$ denotes the probability of occurrence of the symbol $\sigma$ in the sequence $S$. The marginal code length provides a simple encoding mechanism for rules that takes into account the distribution of the individual symbols in the long sequence $S$. Thus, we assign code lengths of $l(S_a, S)$ and $l(S_c, S)$ to the antecedent and succedent of rules. The code lengths $\omega$ are fundamentally different from subsequences since they are real numbers. Nevertheless we can devise an encoding scheme for code lengths inspired on information entropy. If a rule $r$ has code length $\omega(r)$, then storing this value requires a code of length $l(\omega(r), R) = \bar{\omega}(r) \cdot \sum{\mathit{log}(\bar{\omega}(r))}$, where  $\bar{\omega}(r)$ is the normalized code length of rule $r$, and can be calculated as: $\bar{\omega}(r) = \frac{\omega(r)}{\sum_{r' \in R} \omega(r')}$. 
%$l(\omega)  \sum_{(r,w)\in RT}^{ }(
%\sum_{\omega \in a_r}^{ }-log_2(P(v))+
%\sum_{\omega \in c_r}^{ }-log_2(P(v))
%-log_2(\frac{w}{\sum_{(r',w')\in RT}^{ } w'}))$
It follows that the length in bits of a rule table $\mathcal{H}^{\vec{\omega}}(R)$ can be calculated as: 
\begin{equation}
\begin{small}
l(\mathcal{H}^{\vec{\omega}}(R)) = \sum_{r \in R}{l(r\;|\mathcal{H}^{\vec{\omega}}(R))} = \sum_{r : S_a \Rightarrow S_c \in R}{ l(S_a, S) + l(S_c, S) + l(\omega(r), R) 
\end{small}
\end{equation}

\noindent Strictly speaking the term $l(\mathcal{H}^{\vec{\omega}}(R))$ should also consider the price of storing the marginal code lengths, however this factor is constant for a fixed input sequence, and hence irrelevant when mininizing $l(\mathcal{H}^{\vec{\omega}}(R))$.
\commentl{This is also true for $l(S_a, S)$ and $l(S_c, S)$. I could always add this term to the formula.}
%We don't take into account the encoding of the standard ruletable because the corresponding cost is constant in regard of the model, and we suppose the frame of the table to be of large dimension so eventual related cost could be considered constant and discarded as well

\subsubsection{Encoding a Sequence with a Rule Table.}
Given a model in the form of a rule table $\mathcal{H}^{\vec{\omega}}(R)$, we can compute the conditional code length $l(S\;|\;\mathcal{H}^{\vec{\omega}}(R))$ of a sequence $S$ according to the expression: $l(S\;|\;\mathcal{H}^{\vec{\omega}}(R)) = \sum_{1 \ge t \ge |S|}{l(S(t)\;|\;\mathcal{H}^{\vec{\omega}}(R)) }$, i.e., the sum of the joint code lengths of each symbol in the sequence.
We define the \emph{optimal joint code length} of a symbol $S(t)$ in a sequence as $\hat{l}(S(t)\;|\;\mathcal{H}^{\vec{\omega}}(R)) = l(R_{\Vdash}\;|\;S(t))$. In other words, $\hat{l}$ is a function of  the code lengths of the rules that \emph{apply} at position $t$, namely, the rules that correctly predict $S(t)$ based on $S(1, t-1)$, i.e., the previous elements of the sequence. In a setting where we aim at predicting $S(t)$ solely from the model, we only know the rules $R_{\vdash} = \{r \vdash_{t-1} S\}$ that trigger at position $t-1$. From this observation, it follows that: 
\begin{equation}
l(S(t)\;|\;\mathcal{H}^{\vec{\omega}}(R)) = l(R_{\vdash}\;|\;S(t))    
\end{equation}
Since $R_{\vdash} \supset R_{\Vdash}$\footnote{Both sets contain the singleton rules and cannot be equals because only one singleton rule can apply at a given position.}, this code length actually includes the optimal code of $S(t)$ plus the code lengths of the triggering rules that did not correctly predict $S(t)$. This also means that:
\begin{equation}
l(\mathcal{H}^{\vec{\omega}}(R_{\vdash})) - \hat{l}(\mathcal{H}^{\vec{\omega}}(R_{\Vdash})) > 0
\end{equation}
We call this difference the \emph{correction error} of $\mathcal{H}^{\vec{\omega}}(R)$ for $S(t)$ and we denote it by $\delta(S(t)\;|\;\mathcal{H}^{\vec{\omega}}(R))$. This metric quantifies the accuracy of a rule table in bits at predicting $S(t)$ from $S(1, t-1)$. Finally, we need a mechanism to aggregate the code lengths of a set of rules $R'$. We propose the function \emph{LSE} for this purpose:
$$l(\mathcal{H}^{\vec{\omega}}(R')) = LSE(\{-\omega(r'):  r' \in R'\}) = \mathit{log}_2(\sum_{r' \in R'}{2^{-\omega(r')}})$$

%$l(S\;|\;\mathcal{H}^{\vec{\omega}}(R))$$
%this code length must be adjusted to account for the rules $\{r \vdash_t S\}$ that effectively \emph{apply} at position $t$. This analysis brings us to the following formula: whose antecedents match at position $t$
% The length of this joint code obeys the following formula: 
%We then use those information to compute the probability of the next symbol S[t+1] as the ratio of the weight sum of triggered rules having correctly predicted this symbol on the weight sum of triggered rules
%$$l(S(t)\;|\;\mathcal{H}^{\vec{\omega}}(R)) = \mathit{log}_2(\sum_{r \vdash_t S}{2^{\omega(r)}}) - \mathit{log}_2(\sum_{r' \Vdash_t S}{2^{\omega(r')}}) $$
%\begin{small}
%\begin{equation}
%l(S(t)\;|\;\mathcal{H}^{\vec{\omega}}(R)) = \mathit{LSE}_2(\{-\omega_r:  r \vdash_t S\}) - \mathit{LSE}_2(\{ -\omega_{r'} : r' \Vdash_t S\}) 
%\end{equation}
%\end{small}
\noindent The expression $\mathit{LSE}_2(x_1, \dots, x_n)$ is the (log base 2 version of the) LogSumExp function. The selection of \emph{LSE} as aggregation function responds to the fact that code lengths are derived from probabilities in a logarithmic space. 
%The selection of the \emph{LSE} 
%$\frac{
%\sum_{0<t'<t}{ } \sum_{r\in RT, |c_r|>t-t', r is applying at the instant t'}{ } w
%}{
%\sum_{0<t'<t}{ } \sum_{r\in RT, |c_r|>t-t', r is triggering at the instant t'}{ } w
%}
%$
%And then by entropic encoding the length of the sequence S knowing the model RT is :
%$L(S|RT) = \prod_{1<=t<N}^{ } -log_2(P(S[t]|S[1,t+1], RT))$


\subsection{Algorithm}
\label{subsec:cossu}

\begin{algorithm}
\caption{\algCossu{}: finding a compact set of sequential rules}
\label{alg:cossu}
\KwIn{a long sequence $S$ of elements over an alphabet $\Sigma$} 
\KwOut{a compact set of sequential rules $R$}
    $\mathscr{S} := \mathit{closed\text{-}sequence\text{-}mining}(S)}$ \\ 
    $\mathscr{R} := \mathit{rule\text{-}mining}(\mathscr{S})$ \\
    $\mathscr{R} := \{ r \in \mathscr{R}\downarrow^{g(r)} : g(r) > 0 \}$ \\
    $R := \Psi(\Sigma)$ \\
    $\mathscr{R} := \mathscr{R} \setminus \Psi(\Sigma)$ \\
    %$\hat{\vec{\omega}} := \{ r \in R : \frac{s(r) + 1}{\sum_{r \in R}{s(r) + 1}}  \} $ \\
    $\hat{\vec{\omega}} := \textit{argmin}_{\vec{\omega}} l(\mathcal{H}^{\vec{w}}(R')) + l(S|\mathcal{H}^{\vec{w}}(R'))$ \\
    $\hat{\lambda} := l(\mathcal{H}^{\hat{\vec{w}}}(R)) + l(S|\mathcal{H}^{\hat{\vec{w}}}(R))$ \\
    %$\hat{\vec{\omega}} = \mathds{1}^{|R|}$ \\
    %$\vec{\omega} \textit{argmin}_{\vec{\omega}} \mathcal{H}^{\vec{w}}(R) = } 
    \ForEach{$r \in \mathscr{R}$}{
      $R' := R \cup \{ r \} $ \\
      $\hat{\vec{\omega}} := \textit{argmin}_{\vec{\omega}} l(\mathcal{H}^{\vec{w}}(R')) + l(S\;|\;\mathcal{H}^{\vec{w}}(R'))$ \\
      $\lambda := l(\mathcal{H}^{\hat{\vec{w}}}(R')) + l(S\;|\;\mathcal{H}^{\hat{\vec{w}}}(R'))$ \\
      \If{$\lambda < \hat{\lambda}$}{
         $R := R'$ \\
         $\hat{\lambda} := \lambda$\\
      }
      XXX POSTPRUNING OF RULES BECOMING USELESS
    }
    \Return $R$
\end{algorithm}

\noindent Algorithm~\ref{alg:cossu} provides an outline of \algCossu{}. The algorithm takes a sequence $S$ (over an alphabet $\Sigma$) as input and returns a set $R$ of rules mined from $S$. \algCossu{} operates in two phases: a rule construction stage (lines 1-3) finds a large set $\mathscr{R}$ of candidate rules $r: S_a \Rightarrow S_c$ that are then evaluated by a MDL-oriented selection phase (lines 4-14). The selection phase returns a subset $R \subseteq \mathscr{R}$ of rules with good compression performance on the input sequence $S$. We describe these two phases in the following.

\subsubsection{Rule Construction.} \algCossu{} starts by extracting a set of candidate rules $r: S_a \Rightarrow S_c$ from $S$. This is achieved by first applying standard sequence mining techniques to find all closed frequent subsequences from the input sequence $S$ (line 1 in Algorithm~\ref{alg:cossu}). We say a subsequence $S'$  is frequent in $S$ if $s(S') \ge 2$. Furthermore, $S'$ is closed in $S$ if there is no supersequence $S'' \sqsupset S'$ in $S$ such that $\textbf{s}(S'') = \textbf{s}(S')$. Closed subsequences encode the longest co-occurrences of symbols observed in a long sequence. For example, given 
$S = \langle abceabcade \rangle$ and $S' = \langle ab \rangle$ with support $\textbf{s}(S')=2$, we say that $S'$ is not closed in $S$ because  $S'' = \langle abc \rangle \sqsupset S'$ has also support 2. The sequence $S''$, on the contrary, is the only frequent closed sequence in our example. Line 2 leverages the observation that we can generate sequential rules from a sequence $S$ by considering all possible partitionings of $S$ into an antecedent and a non-empty consequent. Our example sequence $S'' = \langle abc \rangle$ produces the candidate rules $ \mathscr{R} = \{ \emptyset \Rightarrow abc,  a \Rightarrow bc, ab\Rightarrow c \}$. In line 3, \algCossu{} sorts the candidate rules by descending \emph{compression gain} $g(r)$ and removes those with non-positive gain. The compression gain is an estimate of the utility of rule $r$ at compressing $S$ and corresponds to the following formula:
\begin{equation}
    g(r) = c(r) \cdot s(r) \cdot l(S_c) - (l(S_a) + l(S_c))
\end{equation}
\noindent The product $c(r) \cdot s(r)$ is the number of times rule $r$ correctly predicts its consequent, so to say, the number of times the code of rule $r$ can be used to encode symbols in $S$. This number is multiplied by the rule's \emph{estimated code length} $l(S_c) = \sum_{\sigma \in S_c}{p(\sigma) \cdot \mathit{log}(p(\sigma))}$. Recall that at this stage, we do not know the joint code length of the rule's consequent, thus we can only approximate it by means of the sum of its marginal code lengths. 
%The first term of $g(r)$ estimates the number of bits saved by compressing $S$ by means of $r$, thus to estimate the compressing gain, we need to account for the price of storing $r$ in the rule table. This is the purpose of the second term $l(S_a)+l(S_c)$. 
The second term $l(S_a)+l(S_c)$ is an estimation of the price of storing $r$ in the rule table. In this way, the rule construction stage provides a set of candidate rules with positive compression potential: rules such that its usage in the data outweights its contribution to the model's complexity. \commentl{I will develop our example.}


\subsubsection{Model selection.}
In our setting a model consists of a set of sequential rules $R$ and their corresponding code lengths, all stored in a rule table $\mathcal{H}^{\vec{w}}(R)$. This table allows us to calculate the number of bits needed to encode the input sequence $S$ with the rules. The challenge of \algCossu{} is to find $\mathcal{H}^{\vec{w}}(R)$ such that Equation~\ref{eq:mdl} is minimized. Alas, this problem is intractable as we are confronted with a space of $2^{|\mathscr{R}|}$ potential models for a set $\mathscr{R}$ of candidate rules. For this reason \algCossu{} resorts to a greedy exploration. Lines 4-7 initialize the exploration.
In line 4 the model is bootstrapped with the singleton rules (removed from the set of candidates in line 5). Having fixed a set of rules, line 6 calculates its optimal code lengths $\vec{\omega}$ in order to build an initial rule table $\mathcal{H}^{\hat{\vec{w}}}(R)$. Line 7 calculates the compression performance of this initial model in the data.  
%\begin{enumerate}
%    \item The optimal code lengths $\vec{\omega}$ of the rules in $R$. This allows us to construct a model $\mathcal{H}^{\vec{w}}(R)$ that we can use to compress the input sequence $S$. This also allow us to calculate the size of the model, i.e., $L(\mathcal{H}^{\vec{w}}(R))$
%    \item The number of bits of $S$ when encoded with $ \mathcal{H}^{\vec{w}}(R)$, namely $L(\mathcal{H}^{\hat{\vec{w}}}(R'))$.
%\end{enumerate}
The exploration starts in line 8. At each step, \algCossu{} adds the rule $r$ with the highest gain $g(r)$ from the set of candidates (line 9) and then calculates the resulting rule table of $R \cup \{ r \} $ in line 10. 
The compression performance of this rule table is calculated in line 11. The rule $r$ is accepted if its inclusion in the rule table reduces the number of bits required to compress the input sequence $S$ (lines 12-14). The process continues until all rules have been explored.


\subsubsection{Optimizing the Weights.}

Given a set of candidate rules $R$, Algorithm~\ref{alg:cossu} must find the set of optimal weights that minimize Equation~\ref{eq:mdl} (lines 6 and 10). From Section~\ref{subsec:rule-encoding} (Eq~X and Y) we know this function has the following form:

\begin{small}
$$ f(S, \mathcal{H}^{\vec{w}}(R)) = \sum_{r \in R}{ l(r\;|\;\mathcal{H}^{\vec{\omega}}(R)) }  + \sum_{1 \le t \le |S|}{ l(\mathcal{H}^{\vec{\omega}}(R_{\vdash})\;|\;t)} $$
\end{small}
Our goal is to find the set of weights $\vec{\hat{\omega}}$ that minimize $f$. Nevertheless,
we do not work directly on this expression, but build upon two observations to simplify it: (i) some of the terms in $f$ do not depend on $\vec{\omega}$, and (ii) in practice our goal is to minimize the correction error of the rule table. Accounting from these observations leads us to the following optimization problem:

$$ \hat{\vec{w}} = \mathit{argmin}_w \sum_{r \in R}{ l(\omega(r)\;|\;R)}  + \sum_{1 \le t \le |S|}{ \delta(S(t)\;|\;\mathcal{H}^{\vec{\omega}}(R))} $$

XXX Briefly explain optimization method. Only first iteration of Powell's method $\Rightarrow$ golden section search on each weight

%\noindent We highlight that we do not need to account for the second term

%\begin{small}
%$$ f(S, \mathcal{H}) = \sum_{r \in R}{ l(r) } + \sum_{1 \le t \le |S|}{l(\mathcal{H}^{\vec{\omega}}(R_{\vdash} \setminus R_{\Vdash}))} $$
%\end{small}




